Round and Communication Efficient Graph Coloring

In the context of communication complexity, we explore protocols for graph coloring, focusing on the vertex and edge coloring problems in $n$-vertex graphs $G$ with a maximum degree $\Delta$. We consider a scenario where the edges of $G$ are partitioned between two players. Our first contribution is a randomized protocol that efficiently finds a $(\Delta + 1)$-vertex coloring of $G$, utilizing $O(n)$ bits of communication in expectation and completing in $O(\log \log n \cdot \log \Delta)$ rounds in the worst case. This advancement represents a significant improvement over the work of Flin and Mittal [Distributed Computing 2025], who achieved the same communication cost but required $O(n)$ rounds in expectation, thereby making a significant reduction in the round complexity. Our second contribution is a deterministic protocol to compute a $(2\Delta - 1)$-edge coloring of $G$, which maintains the same $O(n)$ bits of communication and uses only $O(1)$ rounds. We complement the result with a tight $\Omega(n)$-bit lower bound on the communication complexity of the $(2\Delta-1)$-edge coloring problem, while a similar $\Omega(n)$ lower bound for the $(\Delta+1)$-vertex coloring problem has been established by Flin and Mittal [Distributed Computing 2025]. Our result implies a space lower bound of $\Omega(n)$ bits for $(2\Delta - 1)$-edge coloring in the $W$-streaming model, which is the first non-trivial space lower bound for edge coloring in the $W$-streaming model.

==> archive.tex <==
% \subsection{Preliminary}
% If we denote: $e_i = e^{-\frac{\Delta}{2^{2i + 4}}}$, and $e_i = e_{i + 1}^4$.

% If $t \leq \log \log \Delta$, then $e_t \leq e^{-\frac{\Delta}{2^{2 \log \log \Delta + 4}}} = e^{-\frac{\Delta}{16 \log^2 \Delta}} < \frac{1}{e}$

% Thus, $e_{i - 1} < e_{i} \cdot e$ with every $i < \log \log \Delta$. Then $\sum_{i = 0}^{t} e^{-\frac{\Delta}{2^{2i + 4}}} = \sum_{i = 0}^{t} e_i < \frac{e}{e - 1} \cdot e_t$ if $t < \log \log \Delta$.

% \subsection{Random color trial}
% We can assume that each node has degree $\Delta$. We can add dummy edges to the graph and if the algorithm still provide a valid coloring for the new graph, it will be a valid coloring for the old graph also.

% In each round, every node sleep with probability $1/2$ and awake with probability $1/2$ then pick a color uniformly at random from the set of $\Delta$ colors. If there is no neighbor of the node pick the same color, it will permanently fix to that color. That node is marked as "done", otherwise, it will be marked as "active".

% We want to prove that after $\log \log n$ rounds:
% \begin{itemize}
%     \item There are $O(\frac{n}{\log n})$ active nodes in expectation.
%     \item The bits complexity is $O(n)$ bits in expectation.
%     \item The round complexity is $O(\log \Delta)$ in the worst case.
% \end{itemize}

% \begin{lemma}
%     The probability that the active node marks itself as "done" in the next round is at least $\frac{1}{2e}$.
% \end{lemma}

% \begin{proof}
%     Half of the time the node will awake a pick a color. The probability that one of its neighbors is awake and pick the same color is $\frac{1}{2 \Delta}$. Thus, the probability that the node successfully pick a color in each round is at least
    
%     $$\frac{1}{2} (1 - \frac{1}{2 \Delta})^\Delta \geq \frac{1}{2} (1 - \frac{1}{2 \Delta})^{2 \Delta - 1} \geq \frac{1}{2e}$$
% \end{proof}

% \begin{lemma}
%     In round $i$, if $X_i$ is the number of active nodes. We claim that $E[X_i] \leq n \cdot (1-\frac{1}{2e})^{i}$.
% \end{lemma}

% \begin{proof}
%     It the first round all nodes have $\Delta$ active neighbor which means $X_0 = n$. By lemma 1.1, we have that $E[X_i] \leq n \cdot (1-\frac{1}{2e})^{i}$.
% \end{proof}

% Thus, we can proved the first claim. Recall the binary search method from the previous paper, in each round, for two parties to sample an \emph{available} color for each node, if $k$ is the number of available remaining palette, it requires $O(\log^2 \frac{\Delta}{k})$ bits. Thus, if in round $i$, the node has $k'$ number of active neighbor, then sampling a color only requires at most $O(\log^2 \frac{\Delta}{k'})$.

% We call the node "rich" if in round $i$ it is active and has at least $\frac{\Delta}{2^{2i}}$ active neighbor. We call the node "poor" if it is active but not "rich".

% \begin{lemma}
%     In round $i$, the probability that the "rich" node become "poor" is less than $e^{-\frac{\Delta}{2^{2i+4}}}$.
% \end{lemma}

% \begin{proof}
%     In round $i$, we will calculate what is the probability that the "rich" node become "poor" in that round. 
    
%     First, we will bound the probability that less than a quater of its active neighbor sleep in that round by Chenoff. Since the "rich" node has at least $\frac{\Delta}{2^{2i}}$ number of active neighbor in round $i$, and each neighbor sleep with probability $1/2$ independently. Let $X$ be the number of active neighbor sleep in the next round. We have that $E[X] \geq \frac{\Delta}{2^{2i + 1}}$. By Chenoff bound, the probability that less than one forth of the active neighbor sleep is:

%     $$\Pr[X \leq (1 - \frac{1}{2})\frac{\Delta}{2^{2i + 1}}] \leq \Pr[X \leq (1 - \delta)\mu] \leq e^{-\frac{\delta^2 \mu}{2}} \leq e^{-\frac{\Delta}{2^{2i + 4}}}$$

%     Moreover, if more than a quarter of its active neighbor sleep in that round, the node cannot become "poor". Thus, the probability that the the "rich" node become "poor" in round $i$ is at most $e^{-\frac{\Delta}{2^{2i + 4}}}$.
% \end{proof}

% \begin{corollary}
%     Let $Z_i$ be the number of "rich" node become "poor" in round $i$. We have that $E[Z_i] \leq n \cdot e^{-\frac{\Delta}{2^{2i + 4}}}$.
% \end{corollary}

% \begin{lemma}
%     In round $i$, if $Y_i$ is number of "poor" nodes, then $E[Y_i] \leq \frac{e}{e - 1} \cdot e_t$.
% \end{lemma}

% \begin{proof}
%     $$E[Y_i] \leq \sum_{i = 0}^{i} E[Z_i] = \sum_{i = 0}^{t} e^{-\frac{\Delta}{2^{2i + 4}}} \leq \frac{e}{e - 1} \cdot e_t$$
% \end{proof}

% Now, we are ready to bound the bits complexity. Consider the first $t = \log \log \Delta$ rounds, since the number of "rich" nodes is upper bounded by the number of active nodes, we have that the total bits complexity in expectation is upper bounded by:

% \begin{align*}
%     \sum_{i = 0}^t E[X_i] \cdot O\left(\log \frac{\Delta}{\frac{\Delta}{2^{2i}}}\right) 
%     &+ E[Y_i] \cdot O(\log \Delta) \\
%     &\leq \sum_{i = 0}^t n \cdot \left(1-\frac{1}{2e}\right)^{i} \cdot O(i) + \frac{e}{e - 1} \cdot e_i \cdot O(\log \Delta) \\
%     &\leq O(n) + \frac{e}{(e - 1)}^2 \cdot e_t \cdot O(\log \Delta) \\
%     &\leq O(n) + \frac{e}{(e - 1)}^2 \cdot e^{-\frac{\Delta}{16 \log^2 \Delta}} \cdot O(\log \Delta) \\
%     &\leq O(n) + \frac{e}{(e - 1)}^2 \cdot e^{-\frac{\Delta}{16 \log^2 \Delta} + O(\log \log \Delta)} \\
%     &\leq O(n) + \frac{e}{(e - 1)}^2 \text{ with large enough } \Delta
% \end{align*}

% Let $c = 1 - \frac{1}{2e}$. Recall that the expected number of active nodes is $E[X_t] = n \cdot c^t$. To sample colors in each round, it costs $O(\log \Delta)$ bits in the worst case. Thus, the total bits complexity after the first $t = \log \log \Delta$ rounds is at most:

% \begin{align*}
%     (E[X_t] + E[X_{t+1}] + \cdots) \cdot O(\log \Delta) 
%     &= n \cdot c^t \cdot \frac{c}{1 - c} \cdot O(\log \Delta) \cdot O(\log \Delta) \\
%     &\leq O\left( \frac{n}{\log \Delta} \right) \cdot O(\log \Delta) \\
%     &= O(n)
% \end{align*}

% Thus, we can conclude that the total bit complexity is $O(n)$ in expectation.


% @inproceedings{assadi2019sublinear,
%   title={Sublinear algorithms for {$(\Delta+ 1)$} vertex coloring},
%   author={Assadi, Sepehr and Chen, Yu and Khanna, Sanjeev},
%   booktitle={Proceedings of the Thirtieth Annual ACM-SIAM Symposium on Discrete Algorithms {(SODA)}},
%   pages={767--786},
%   year={2019},
%   organization={SIAM}
% }

% @inproceedings{halldorsson2022near,
%   title={Near-optimal distributed degree + 1 coloring},
%   author={Halld{\'o}rsson, Magn{\'u}s M and Kuhn, Fabian and Nolin, Alexandre and Tonoyan, Tigran},
%   booktitle={Proceedings of the 54th Annual ACM SIGACT Symposium on Theory of Computing {(STOC)}},
%   pages={450--463},
%   year={2022}
% }

% @inproceedings{10.1145/3662158.3662796, author = {Flin, Maxime and Mittal, Parth}, title = { {$(\Delta+ 1)$} Vertex Coloring in {$O(n)$} Communication}, year = {2024}, isbn = {9798400706684}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/3662158.3662796}, doi = {10.1145/3662158.3662796}, booktitle = {Proceedings of the 43rd ACM Symposium on Principles of Distributed Computing {(PODC)}}, pages = {416–424}, numpages = {9}, keywords = {coloring, communication complexity, sparsification}, location = {Nantes, France}}

% @article{dubhashi22concentration,
%   title={Concentration of measure for the analysis of randomised algorithms, 2005},
%   author={Dubhashi, Devdatt and Panconesi, Alessandro},
%   journal={Manuscript. Available from http://http://www.dsi.uniroma1.it/ale/papers.html},
%   volume={22},
%   pages={24},
%   year={2005}
% }

% The previous work claimed that a randomized protocol exists to solve k-Slack-Int with \( O(\log^2(m/k)) \) bits of communication in expectation. They employed several noteworthy techniques:

% \begin{enumerate}
%     \item \textbf{Deterministic Protocol:} There is a \emph{deterministic} protocol that solves \cref{prob:ksi} with \( O(\log^2(m)) \) bits of communication for any \( k > 1 \). This protocol uses binary search to locate an element in the set by partitioning it.
    
%     \item \textbf{Randomized Algorithm:} The randomized algorithm operates by guessing the value of \( k \) through binary search. For each guess of \( k \), elements are sampled with probability \( p \) as a function of $k$. With an appropriately chosen \( p \), the set of sampled elements \( S \) will include an element not in \( X \) or \( Y \) with a significant probability. If such an element exists in \( S \), the deterministic protocol is then used to identify it.
    
%     \item \textbf{Choice of \( p \):} The deterministic protocol requires \( O(\log^2(|S|)) \) bits of communication. To ensure that \( S \) has a size of \( \text{poly}(m/k) \), it is restricted to \( p \in \left\{ \frac{1}{k}, \frac{m}{k^2}, \ldots \right\} \). While \( p = \frac{1}{k} \) might not be sufficient,  choosing \( p = \frac{m}{k^2} \) is effective, as it increases the likelihood of a stronger condition of \( S \) containing an element not in \( X \) or \( Y \).
    
%     \item \textbf{Stronger Condition:} A stronger but simpler condition is used to ensure that \( S \) contains the desired element. Specifically, if \( |S \cap X| + |S \cap Y| < |S| \), the set \( S \) is guaranteed to include an element not in \( X \) or \( Y \). Checking this condition requires only \( \log |S| \) bits of communication, as the parties exchange \( |S \cap X| \) and \( |S \cap Y| \). With \( p = \frac{m}{k^2} \), this condition is met with constant probability by Chenoff Bound. 
% \end{enumerate}

% We will first compute the upper bound on the expected bits complexity for a single node $v$ to sample colors using \cref{alg:k-Slack-Int} in the $i$th iteration. Let \( C_{i,v} \) be a random variable indicating the communication cost incurred by node \( v \) in that round. Note that the cost is non-zero if and only if node \( v \) is \textsf{active} in the $i$th iteration. Let $A$, $H$ and $L$ be the event that node \( v \) is \textsf{active}, \textsf{high-degree} and \textsf{low-degree}, respectively, in the $i$th iteration.

% The expected cost can be expressed as:

% \begin{align*}
% \E[C_{i,v}] &= \Pr[H] \cdot \E[C_{i,v} \mid H] + \Pr[L] \cdot \E[C_{i,v} \mid L] \\
% &\leq \Pr[A] \cdot \E[C_{i,v} \mid H] + \Pr[L] \cdot O(\log^2 \Delta) \\
% &\leq \left( \frac{23}{24} \right)^i \cdot O(i) + \frac{e}{e - 1} \cdot a_i \cdot O(\log^2 \Delta)
% \end{align*}

% That is because, in the $i$th iteration, the probability that a node $v$ is \textsf{active} is at most $\left(\frac{23}{24}\right)^i$. The expected cost, given that $v$ is \textsf{high-degree}, is $O(i)$. Additionally, the probability that a node $v$ is \textsf{low-degree} is at most $\frac{e}{e - 1} \cdot a_i$. In the worst case, sampling a color takes $O(\log^2 \Delta)$ bits.

% Now, we are ready to bound the expected total bits complexity. Let $C$ denote the total bits complexity. By linearity of expectation, we have that 

% \begin{align*}
% \E[C] & = \sum_v \sum_{i=0}^{t} \E[C_{i,v}] \\
% & \leq n \cdot \sum_{i=0}^{t} \left( \left( \frac{23}{24} \right)^i \cdot O(i) + \frac{e}{e - 1} \cdot a_i \cdot O(\log^2 \Delta) \right) \\
% & = n \cdot \sum_{i=0}^{t} \left( \left( \frac{23}{24} \right)^i \cdot O(i) \right) + n \cdot \sum_{i=0}^{t} \left( \frac{e}{e - 1} \cdot a_i \cdot O(\log^2 \Delta) \right) \\
% & = n \cdot O(1) + n \cdot \left( \frac{e}{e - 1} \right)^2 \cdot a_t \cdot O(\log^2 \Delta) \\
% & < n \cdot O(1) + n \cdot \left( \frac{e}{e - 1} \right)^2 \cdot \frac{1}{\log^2 \Delta} \cdot O(\log^2 \Delta) \\
% & = O(n)
% \end{align*}



% \paragraph{Deferring Edges} 
% Alice and Bob will each use \(\Delta\) colors to color their edges, with their color sets sharing only one \emph{common} \textsf{special} color. To satisfy the condition in \cref{thm:edge_main}, Alice and Bob will \emph{sequentially} mark and remove edges connecting two vertices of degree \(\Delta\) in their respective edge sets. In the remaining subgraph, after marking these edges, there are no connected pairs of vertices of degree \(\Delta\). They will utilize the colors from the other party to color these marked edges and will defer this coloring until both parties have completed coloring the subgraph. Intuitively, it is not difficult to color these marked edges on Alice's side, as there are no incident edges on Bob's side for these edges. It is important to note that marking these edges requires no communication between Alice and Bob.

% \paragraph{Coloring the Subgraph} 
% At this stage, both Alice and Bob have subgraphs in which no pairs of vertices of degree \(\Delta\) are connected. According to the results established in \cref{thm:edge_main}, they can achieve a proper \(\Delta\)-edge-coloring such that every edge \(uv\) receives a color from the set \(\{1, \ldots, \min\{\Delta, 1 + \max\{d(u), d(v)\}\}\}\). We will designate the common \textsf{special} color as the \emph{last} color in both color sets. By the theorem, an edge will be assigned the \textsf{special} color only if at least one of its endpoints has a degree of at least \(\Delta - 1\). We will analyze the various cases in which this color might clash with other party and address them accordingly. 

% Consider two edges having a special color: $uv$ in Alice's graph and $vt$ in Bob's graph. There are several cases:

% \vspace{1em}

% \begin{tabular}{|c|c|c|c|c|}
% \hline
% & Vertex $u$ & Vertex $v$ & Vertex $t$ & Note \\
% \hline
% Case 1    & \(\Delta - 1\) in Alice's  & \(\Delta - 1\) in Bob's   &  & Simple color replace  \\
% \hline
% Case 2    & \(\Delta\) in Alice's  & \(\Delta - 1\) in Bob's   &  &  \\
% \hline
% Case 3    & $\Delta / \Delta - 1$ in Alice's  & \(\Delta\) in Bob's   &  & Impossible \\
% \hline
% Case 4    & $\Delta / \Delta - 1$ in Alice's  & & $\Delta / \Delta - 1$ in Bob's & Sample replacing color  \\
% \hline
% \end{tabular}

% \paragraph{Case 1} Let \(u\) be the vertex of degree \(\Delta - 1\) in Alice's graph, and let \(v\) be the vertex of degree \(\Delta - 1\) in Bob's graph. In this scenario, the edge \(uv\) in Alice's graph is colored with the \textsf{special} color, while there exists an edge adjacent to \(v\) that is also colored with the \textsf{special} color in Bob's graph. This situation can be resolved easily by replacing the \textsf{special} color of the edge \(uv\) with one of the remaining colors from Alice's set of \(\Delta - 1\) colors. Since the vertex \(v\) has degree one in Alice's graph, this replacement maintains a proper coloring.

% \paragraph{Case 2} Let \(u\) be the vertex of degree $\Delta$ in Alice's graph, and let \(t\) be the vertex of degree \(\Delta - 1\) in Bob's graph. If there is another edge $us$ in Alice's graph such that $s$ is not a vertex of degree $\Delta - 1$ in Bob, we will 

% \paragraph{Case 4} Let \(u\) be the vertex of degree at least \(\Delta - 1\) in Alice's graph, and let \(t\) be the vertex of degree at least \(\Delta - 1\) in Bob's graph. Note that vertex \(v\) has degree smaller than \(\Delta - 1\) in both party's graph, as this scenario has been addressed in other cases. Initially, they will use \(O(n)\) bits of communication to identify all vertices \(v\) with degree smaller than \(\Delta - 1\) that are incident to the \emph{special} color edge, all within a single round. They will then replace the \textsf{special} color of either edge \(vu\) or \(vt\) with a color from the set of colors belonging to the other party.


% \begin{lemma}
%     There exists a protocol that finds a proper replacement color using an expected \(O(n)\) bits of communication and completes in \(O(\log n)\) rounds with high probability.
% \end{lemma}

% \begin{proof}
% It is straightforward to observe that the degree of vertex \(v\) is at most \(\Delta / 2\) in either Alice's or Bob's graph. They will use another round of communication and \(O(n)\) bits to indicate whether vertex \(v\) has degree at most \(\Delta / 2\) in their respective graphs. Intuitively, using a color from the other party for replacement is easy if the degree of vertex \(v\) in that party's graph is small. If the degree of vertex \(v\) in one party's graph exceeds \(\Delta / 2\), they will replace the \textsf{special} color edge in that party. In the case that the degree of vertex \(v\) is small in both graphs, they will use public randomness to determine which party should replace the \textsf{special} color.

% If Alice needs to replace the \textsf{special} color of edge \(uv\), Alice and Bob will sample a color uniformly at random from Bob's colors using public randomness. Bob will then send a one-bit confirmation indicating whether the color is valid on his side. However, if Alice obtains only \textbf{one} valid color from Bob's available colors for vertex \(v\), this is \emph{insufficient}, as there may be an edge connected to \(u\) in Bob's graph that shares the same color.


% \begin{remark}
%     Note that Bob only knows about vertex \(v\) and is unaware that \(uv\) is the \textsf{special} colored edge in Alice's graph. Consequently, it is challenging for Alice to determine the color of the edge incident to \(u\) in Bob's graph. If Bob sends the color of this edge, it would require \(O(\log \Delta)\) bits of communication for each vertex \(u\). Thus, the total bit complexity would be \(O(n \log \Delta)\), exceeding our target.
% \end{remark}

% To overcome this issue, Alice and Bob will first agree on a grouping of colors in their respective sets (excluding the \textsf{special} color). The colors can be divided arbitrarily into three groups of roughly equal size (approximately \(\Delta/3\)), and they both know this classification. Alice will sample Bob's colors until she obtains two colors from two different groups that are \emph{valid} (i.e., not used by edges incident to \(v\) in Bob's graph).

% The probability that Alice acquires the first \textit{valid} color is at least a constant since the number of colors occupied by edges incident to \(v\) in Bob's graph is at most \(\Delta / 2\). After obtaining the first \textit{valid} color, the probability of acquiring a second \textit{valid} color from a different group is also at least a constant because the number of colors in the first group is at most \(1 + \Delta / 3\). Thus, the expected number of rounds and one-bit confirmations Bob needs to send is upper-bounded by a constant.

% Considering the round complexity, they will sample colors for all such vertices \(v\) in parallel. The probability that the procedure completes within two rounds for each vertex is at least another constant. Since the number of such vertices \(v\) is \(O(n)\), the procedure will finish in \(O(\log n)\) rounds of communication with high probability.

% Finally, Alice and Bob will exchange the lists of vertices with degree \(\Delta - 1\). For each vertex \(u\) with degree \(\Delta - 1\) in Alice's graph, Bob will send the group number of the color of the edge incident to \(u\) in his graph. Alice will then select a color from a different group to replace the color of edge \(uv\). This step requires \(O(n)\) bits in a constant number of communication rounds.
% \end{proof}




% \paragraph{Algorithm Description} 


% \paragraph{Problem definition} In graph $G$ with $n$ vertex, the edges are partitioned to two parties adversarially. Two parties need to color the edges using $2\Delta - 1$ colors. We examine $2\Delta - 1$ colors since this is the minimum numbers of color needed for greedy algorithm. We want to have a algorithm with expected bit complexity of $O(n)$. It is fine if a party does not know about the color of an edge in other party since even transfer all the colors of all edges in one party need $O(\log \Delta \cdot n^2$) bits of communication. 
% \hung{This can be polished added into preliminary, or I think it is already been added.}
